Unified Graph Networks (UGN): A Deep Neural Framework for Solving Graph Problems

Deep neural networks have enabled researchers to create powerful generalized frameworks, such as transformers, that can be used to solve well-studied problems in various application domains, such as text and image. However, such generalized frameworks are not available for solving graph problems. Graph structures are ubiquitous in many applications around us and many graph problems have been widely studied over years. In recent times, there has been a surge in deep neural network based approaches to solve graph problems, with growing availability of graph structured datasets across diverse domains. Nevertheless, existing methods are mostly tailored to solve a specific task and lack the capability to create a generalized model leading to solutions for different downstream tasks. In this work, we propose a novel, resource-efficient framework named \emph{U}nified \emph{G}raph \emph{N}etwork (UGN) by leveraging the feature extraction capability of graph convolutional neural networks (GCN) and 2-dimensional convolutional neural networks (Conv2D). UGN unifies various graph learning tasks, such as link prediction, node classification, community detection, graph-to-graph translation, knowledge graph completion, and more, within a cohesive framework, while exercising minimal task-specific extensions (e.g., formation of supernodes for coarsening massive networks to increase scalability, use of \textit{mean target connectivity matrix} (MTCM) representation for achieving scalability in graph translation task, etc.) to enhance the generalization capability of graph learning and analysis. We test the novel UGN framework for six uncorrelated graph problems, using twelve different datasets. Experimental results show that UGN outperforms the state-of-the-art baselines by a significant margin on ten datasets, while producing comparable results on the remaining dataset.

==> Latex/FigDef/football_polbooks.tex <==
\begin{figure}[htbp]
\centering
\includegraphics[width=\linewidth]{Latex/images/football.png}
\caption{American College football}
\label{fig:football}
\end{figure}

\begin{figure}[htbp]
\centering
\includegraphics[width=\linewidth]{Latex/images/polbooks.png}
\caption{Books about US politics}
\label{fig:polbooks}
\end{figure}

==> Latex/FigDef/hcp.tex <==
\begin{figure}[htbp]
\centering
\includegraphics[width=\linewidth]{Latex/images/HCP.png}
\caption{Training process of the model on the HCP dataset}
\label{fig:HCP_training}
\end{figure}

==> Latex/FigDef/karate.tex <==
\begin{figure}[htbp]
\centering
\includegraphics[width=\linewidth]{Latex/images/karate2.png}
\caption{Zachary's karate club with two communities}
\label{fig:karate2c}
\end{figure}

\begin{figure}[htbp]
\centering
\includegraphics[width=\linewidth]{Latex/images/karate4.png}
\caption{Zachary's karate club with four communities}
\label{fig:karate4c}
\end{figure}

==> Latex/FigDef/model_datasets.tex <==
\begin{figure}[t]
\centering
%\vspace{-.2cm}
\includegraphics[width=0.5\textwidth]{Latex/images/UGN_model.png}
\caption{
\small An overview of our proposed UGN framework.
}
\label{fig:arch}
\end{figure}

==> Latex/Tabledef/abls_hcp_karate_tab.tex <==
\begin{comment}
\begin{table*}[htbp]
\parbox{.4\linewidth}{
\centering
\begin{tabular}{||c|c||}
\hline
Method & \makecell{Pearson\\Correlation} \\
\hline\hline
Our Model & \textbf{0.66}\\
Our Model - MTCM & 0.36\\
\hline
\end{tabular}
\caption{Ablation Study on the HCP dataset Motoring task}
\label{tab:abls_HCP}
}
\hfill
\parbox{.6\linewidth}{
\centering
\begin{tabular}{||c|c|c||}
\hline
\diagbox{Method}{Node Acc.} & 2-Community &  4-Community\\
\hline\hline
Our Model & \textbf{1.00} & \textbf{0.93}\\
Our Model - $\mathcal{L}_u$ & 0.91 & 0.87\\
\hline
\end{tabular}
\caption{Ablation Study on the Zachary's karate club dataset}
\label{tab:abls_karate}
}
\end{table*}
\end{comment}

==> Latex/Tabledef/abls_iot60_slashdot_hcp_karate_tab.tex <==
\begin{table*}[htbp]
    \begin{subtable}{.23\linewidth}
      \centering
        \begin{tabular}{||c|c|c||}
        \hline
        \makecell{Decoder\\Type} & \makecell{Node\\Acc.} & \makecell{Edge\\Acc.} \\
        \hline\hline
        MLP & 0.66 & 0.91 \\
        LSTM & 0.84 & 0.95 \\
        BiLSTM & 0.85 & 0.95 \\
        UGN & \textbf{0.94} & \textbf{0.98} \\
        \hline
        \end{tabular}
        \caption{IoT-60}
        \label{tab:abls_IOT60}
    \end{subtable}%
    \begin{subtable}{.3\linewidth}
      \centering
        \begin{tabular}{||c|c||}
        \hline
        Method & \makecell{Edge\\Acc.} \\
        \hline\hline
        UGN & \textbf{0.82}\\
        UGN - SuperNode feature & 0.80\\
        \hline
        \end{tabular}
        \caption{Slashdot}
        \label{tab:abls_Slashdot}
    \end{subtable}%
    \begin{subtable}{.25\linewidth}
      \centering
        \begin{tabular}{||c|c||}
        \hline
        Method & \makecell{Pearson\\Correlation} \\
        \hline\hline
        UGN & \textbf{0.66}\\
        UGN - MTCM & 0.36\\
        \hline
        \end{tabular}
        \caption{HCP Motoring task}
        \label{tab:abls_HCP}
    \end{subtable} 
    \begin{subtable}{.2\linewidth}
      \centering
        \begin{tabular}{||c|c||}
        \hline
        Method & \makecell{Node\\Acc.} \\
        \hline\hline
        UGN & \textbf{1.00} \\
        UGN - $\mathcal{L}_u$ & 0.91 \\
        \hline
        \end{tabular}
        \caption{Zachary's karate club}
        \label{tab:abls_karate}
    \end{subtable}
    \caption{Ablation Study by component replacement and removal on (a) IoT-60 dataset, (b) Slashdot dataset, (c) HCP dataset Motoring task, and (d) Zachary's karate club dataset}
\end{table*}

\begin{comment}
\begin{table}[htbp]
\parbox{\linewidth}{
\centering
\begin{tabular}{||c|c|c||}
\hline
Decoder Type & Node Acc. & Edge Acc. \\
\hline\hline
MLP & 0.66 & 0.91 \\
LSTM & 0.84 & 0.95 \\
BiLSTM & 0.85 & 0.95 \\
UGN & \textbf{0.94} & \textbf{0.98} \\
\hline
\end{tabular}
\caption{Ablation Study on the IoT-60 dataset}
\label{tab:abls_IOT60}
}
\hfill
\parbox{\linewidth}{
\centering
\begin{tabular}{||c|c||}
\hline
Method & Edge Acc. \\
\hline\hline
UGN & \textbf{0.82}\\
UGN - SuperNode feature & 0.80\\
\hline
\end{tabular}
\caption{Ablation Study on the Slashdot dataset}
\label{tab:abls_Slashdot}
}
\hfill
\parbox{\linewidth}{
\centering
\begin{tabular}{||c|c||}
\hline
Method & \makecell{Pearson\\Correlation} \\
\hline\hline
UGN & \textbf{0.66}\\
UGN - MTCM & 0.36\\
\hline
\end{tabular}
\caption{Ablation Study on the HCP dataset Motoring task}
    \label{tab:abls_HCP}
}
\hfill
\parbox{\linewidth}{
\centering
\begin{tabular}{||c|c|c||}
\hline
\diagbox{Method}{Node Acc.} & 2-Community &  4-Community\\
\hline\hline
UGN & \textbf{1.00} & \textbf{0.93}\\
UGN - $\mathcal{L}_u$ & 0.91 & 0.87\\
\hline
\end{tabular}
\caption{Ablation Study on the Zachary's karate club dataset}
\label{tab:abls_karate}
}
\end{table}
\end{comment}

==> Latex/Tabledef/recoms_res_cmp_tab.tex <==
\begin{table*}[htbp]
\centering
\begin{tabular}{||c|c|c|c|c|c|c|c|c||}
\hline
Method & \makecell{GHRS \\\cite{darban2022ghrs}} & \makecell{GLocal-K \\\cite{han2021glocal}} & \makecell{GraphRec \\\cite{rashed2019attribute}} & \makecell{IGMC \\\cite{zhanginductive}} & \makecell{GC-MC \\\cite{berg2017graph}} & \makecell{F-EAE \\\cite{hartford2018deep}} & \makecell{PinSage \\\cite{ying2018graph}} & Our Model \\
\hline\hline
RMSE & \textbf{0.89} & \textbf{0.89} & 0.90 & 0.91 & 0.91 & 0.92 & 0.95 & 1.01\\
\hline
\end{tabular}
\caption{Performance Comparison on the MovieLens-100k dataset}
\label{tab:MovieLens_compare}
\end{table*}

==> Latex/Tabledef/supernode_form_fig_tab.tex <==
\begin{figure*}[htbp]
\begin{subfigure}[H]{0.3\textwidth}
\centering
\includegraphics[width=\textwidth]{Latex/images/supernode.png}
\caption{A graph with 9 nodes and 3 super-nodes}
\label{fig:supernode}
\end{subfigure}
\begin{subfigure}[H]{0.3\textwidth}
\setlength{\tabcolsep}{3pt}
\centering
%\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|}
\begin{tabular}{@{}cc||*{9}{c|}}

\multicolumn{1}{c}{}  &   &\multicolumn{9}{c|}{Nodes}\\
\multicolumn{1}{c}{} & &1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9\\
\hline \hline
\multirow{9}*{\rotatebox{90}{Nodes}} &
1 & \cellcolor{sn1} & \cellcolor{sn1} 1 & \cellcolor{sn1} & \cellcolor{sn2} & \cellcolor{sn2} 1 & \cellcolor{sn2} & \cellcolor{sn3} & \cellcolor{sn3} & \cellcolor{sn3} \\ \cline{2-2}\hhline{~~||*9{-}|}

&2 & \cellcolor{sn1} 1 & \cellcolor{sn1} & \cellcolor{sn1} 1 & \cellcolor{sn2} 1 & \cellcolor{sn2} & \cellcolor{sn2} & \cellcolor{sn3} 1 & \cellcolor{sn3} & \cellcolor{sn3} \\ \cline{2-2}\hhline{~~||*9{-}|}

&3 & \cellcolor{sn1} & \cellcolor{sn1} 1 & \cellcolor{sn1} & \cellcolor{sn2} & \cellcolor{sn2} & \cellcolor{sn2} & \cellcolor{sn3} & \cellcolor{sn3} & \cellcolor{sn3} 1 \\ \cline{2-2}\hhline{~~||*9{-}|}

&4 & \cellcolor{sn1} & \cellcolor{sn1} 1 & \cellcolor{sn1} & \cellcolor{sn2} & \cellcolor{sn2} & \cellcolor{sn2} 1 & \cellcolor{sn3} & \cellcolor{sn3} 1 & \cellcolor{sn3} \\ \cline{2-2}\hhline{~~||*9{-}|}

&5 & \cellcolor{sn1} 1 & \cellcolor{sn1} & \cellcolor{sn1} & \cellcolor{sn2} & \cellcolor{sn2} & \cellcolor{sn2} 1 & \cellcolor{sn3} & \cellcolor{sn3} & \cellcolor{sn3} \\ \cline{2-2}\hhline{~~||*9{-}|}

&6 & \cellcolor{sn1} & \cellcolor{sn1} & \cellcolor{sn1} & \cellcolor{sn2} 1 & \cellcolor{sn2} 1 & \cellcolor{sn2} & \cellcolor{sn3} 1 & \cellcolor{sn3} & \cellcolor{sn3} \\ \cline{2-2}\hhline{~~||*9{-}|}

&7 & \cellcolor{sn1} & \cellcolor{sn1} 1 & \cellcolor{sn1} & \cellcolor{sn2} & \cellcolor{sn2} & \cellcolor{sn2} 1 & \cellcolor{sn3} & \cellcolor{sn3} & \cellcolor{sn3} \\ \cline{2-2}\hhline{~~||*9{-}|}

&8 & \cellcolor{sn1} & \cellcolor{sn1} & \cellcolor{sn1} & \cellcolor{sn2}1 & \cellcolor{sn2} & \cellcolor{sn2} & \cellcolor{sn3} & \cellcolor{sn3} & \cellcolor{sn3} 1 \\ \cline{2-2}\hhline{~~||*9{-}|}

&9 & \cellcolor{sn1} & \cellcolor{sn1} & \cellcolor{sn1} 1 & \cellcolor{sn2} & \cellcolor{sn2} & \cellcolor{sn2} & \cellcolor{sn3} & \cellcolor{sn3} 1 & \cellcolor{sn3} \\ \cline{1-2}\hhline{~~||*9{-}|}
\end{tabular}
\caption{Adjacency Matrix of the Graph}
\label{tab:supernode1}
\end{subfigure}
\begin{subfigure}[H]{0.2\textwidth}
\centering
%\begin{tabular}{|c|c|c|c|}
\begin{tabular}{@{}cc||*{3}{c|}}
\multicolumn{1}{c}{}  &   &\multicolumn{3}{c|}{SuperNodes}\\
\multicolumn{1}{c}{} & & 1 & 2 & 3 \\
\hline \hline
\multirow{9}*{\rotatebox{90}{Nodes}} &
1 & \cellcolor{sn1} 0.33 & \cellcolor{sn2} 0.33 & \cellcolor{sn3} 0.00 \\ \cline{2-2}\hhline{~~||*3{-}|}

&2 & \cellcolor{sn1} 0.67 & \cellcolor{sn2} 0.33 & \cellcolor{sn3} 0.33 \\ \cline{2-2}\hhline{~~||*3{-}|}

&3 & \cellcolor{sn1} 0.33 & \cellcolor{sn2} 0.00 & \cellcolor{sn3} 0.33 \\ \cline{2-2}\hhline{~~||*3{-}|}

&4 & \cellcolor{sn1} 0.33 & \cellcolor{sn2} 0.33 & \cellcolor{sn3} 0.33 \\ \cline{2-2}\hhline{~~||*3{-}|}

&5 & \cellcolor{sn1} 0.33 & \cellcolor{sn2} 0.33 & \cellcolor{sn3} 0.00 \\ \cline{2-2}\hhline{~~||*3{-}|}

&6 & \cellcolor{sn1} 0.00 & \cellcolor{sn2} 0.67 & \cellcolor{sn3} 0.33 \\ \cline{2-2}\hhline{~~||*3{-}|}

&7 & \cellcolor{sn1} 0.33 & \cellcolor{sn2} 0.33 & \cellcolor{sn3} 0.00 \\ \cline{2-2}\hhline{~~||*3{-}|}

&8 & \cellcolor{sn1} 0.00 & \cellcolor{sn2} 0.33 & \cellcolor{sn3} 0.33 \\ \cline{2-2}\hhline{~~||*3{-}|}

&9 & \cellcolor{sn1} 0.33 & \cellcolor{sn2} 0.00 & \cellcolor{sn3} 0.33 \\ \cline{1-2}\hhline{~~||*3{-}|}

\end{tabular}
\caption{Supernode features}
\label{tab:supernode2}
\end{subfigure}
%\captionlistentry{}
\caption{Supernode construction}
\label{supernodeConstruction}
\end{figure*}

==> Latex/sections/related_work.tex <==
\citet{guo2019deep} proposed a generic, end-to-end framework for joint node and edge attributes prediction, which is a need for realworld applications such as malware confinement in IoT networks and structural-to-functional network translation. Their novel edge translation path is generic, which is proven to be a generalization of the existing topology translation models. Authors also proposed a spectral graph regularization based strategy on their non-parametric graph Laplacian in order to learn and maintain the consistency of the predicted nodes and edges.

\citet{bruna2014spectral} first introduced the spectral graph convolutional neural networks, and then it was extended by \citet{defferrard2016convolutional} using fast localized convolutions, which is further approximated by \citet{DBLP:conf/iclr/KipfW17} for an efficient architecture for a semi-supervised setting. \citet{li2018diffusion} proposed a Diffusion Convolution Recurrent Neural Network (DCRNN) for traffic forecasting which incorporates both spatial and temporal dependency in the traffic flow. \citet{Yu2018SpatioTemporalGC} formulated the node attributes prediction problem of graphs based on the complete convolution structures. \citet{9737289} tackled graph topology translation problem by proposing a generative model consisting of a graph translator with graph convolution and deconvolution layers and a new conditional graph discriminator. \citet{sun2019graph} proposed a graphRNN based model which generates a graph’s topology based on another graph.

\citet{wang2020edge2vec} proposed edge-based graph embedding (edge2vec) to map the edges in social networks directly to low-dimensional vectors considering an important property of social networks, i.e., the networka are sparse, and hence the average degree of nodes is bounded. Edge2vec takes both the local and the global structure information of edges into consideration to preserve structure information of embedded edges as much as possible. To achieve this goal, edge2vec ingeniously combines the deep autoencoder and Skip-gram model through a well-designed deep neural network.

\citet{perozzi2014deepwalk} proposed DeepWalk to employ the truncated random walks and obtain the context information of nodes. \citet{grover2016node2vec} proposed Node2vec to improve DeepWalk through replacing the truncated random walks with a new search strategy which combines the property of Breadth First Search (BFS) and Depth First Search (DFS). \citet{tang2015line} proposed LINE to consider the neighborhood of a node as its context. \citet{cao2015grarep} proposed GraRep to extend LINE by considering the indirect neighbors, but it suffers from the length of embedding vectors. Discriminative Deep Random Walk (DDRW) and max-margin DeepWalk (MMDW) proposed by \citet{li2016discriminative} and \citet{tu2016max} respectively try to jointly optimize the classifier and the embedding model. RSDNE proposed by \citet{wang2018rsdne} approximately guarantees intra-class similarity and inter-class dissimilarity, obtaining favorable performance in both the general and zero-shot graph embedding problems.

\citet{waskiewicz2012friend} divided the static community detection methods into four broad categories as spectral methods, methods based on statistical inference, methods based on optimization and methods based on dynamics. Spectral methods use spectral properties like eigen value spectrum of the matrix representations (e.g., adjacency matrix, Laplacian matrix, modularity matrix etc.) of networks to detect communities.  The works of \citet{newman2006finding}\cite{newman2013spectral} can be given as examples of spectral methods. Methods based on statistical inference generally adopts an ordinary approach to fit data to a generative network model. Most popular generative model with communities for networks is Stochastic Block Model (SBM). The works of \citet{come2015model}, and \citet{newman2016estimating} can be given as examples of statistical inference-based community detection methods. Methods based on optimization try to find a maximum or minimum of a quality function that shows the quality of community structure. Most popular quality function is modularity proposed by \citet{newman2004finding}. Modularity is a concept depending on the maximization of difference between actual network and another form of actual network that have randomly destroyed community structure. The methods proposed by \citet{clauset2005finding}, and \citet{lancichinetti2011limits} can be given as examples of methods based on optimization. Methods based on dynamics uses running dynamics of the networks like diffusion, random walk and spin dynamics to detect community structure in a network. The works of \citet{reichardt2006statistical}, and \citet{rosvall2008maps} can be given as examples for methods based on dynamics.

\begin{comment}
\textcolor{magenta}{The matrix completion problem has been studied using GNNs. \citet{monti2017geometric} developed a multi-graph CNN (MGCNN) model to extract user and item latent features from their respective nearest-neighbor networks. \citet{berg2017graph} proposed graph convolutional matrix completion (GC-MC) which directly applies a GNN to the user-item bipartite graph to extract user and item latent features using a GNN. Although using GNNs for matrix completion, all these models are still transductive – MGCNN requires graph Laplacians which do not generalize to new graphs, while GC-MC uses one-hot encoding of node IDs as initial node features, thus cannot generalize to unseen users/items. A recent inductive graph-based recommender system, PinSage (\citet{ying2018graph}), uses node content as initial node features (instead of the one-hot encoding in GC-MC), and is successfully used in recommending related pins in Pinterest. \citet{zhanginductive} proposed an Inductive Graph-based Matrix Completion (IGMC) model which trains a graph neural network (GNN) based purely on 1-hop subgraphs around (user, item) pairs generated from the rating matrix and maps those subgraphs to their corresponding ratings.}
\end{comment}

\textcolor{magenta}{Knowledge graph embedding is an active research topic with many different methods. They can be categorized based on the interaction mechanisms and the computation of the matching score. Tensor-decomposition-based models adapt tensor representation formats such as CP format, Tucker format, and block term format to represent the knowledge graph data tensor (\citet{kolda2009tensor}). They make up most of recent SOTA models such as ComplEx (\citet{trouillon2016complex}), SimplE (\citet{kazemi2018simple}), TuckER (\citet{balavzevic2019tucker}), and MEIM (\citet{DBLP:conf/ijcai/TranT22}). They often achieve good trade-off between efficiency and expressiveness. Neural-network-based models use a neural network to compute the matching score, such as ConvE (\citet{dettmers2018convolutional}) using convolutional neural networks, CompGCN (\citet{vashishthcomposition}) using graph convolutional networks. These models are generally more expensive but not always get better results than tensor-decomposition-based models. Translation-based models use geometrical distance to compute the matching score, with relation embeddings act as the translation vectors, such as TransE (\citet{bordes2013translating}). These models are efficient and intuitive, but they have limitations in expressive power (\citet{kazemi2018simple}). There are several ways to use orthogonality in knowledge graph embedding, such as RotatE (\citet{sunrotate}) using complex product, Quaternion (\citet{tran2019analyzing}) and QuatE (\citet{zhang2019quaternion}) using quaternion product, GCOTE (\citet{tang2020orthogonal}) using the Gram Schmidt process, and RotH (\citet{chami2020low}) using the Givens matrix.}

Our model is unique in terms of scalability and genericness.
\textcolor{magenta}{
%\begin{enumerate}
%\item 
(i) We experimented with smaller graphs containing 20-60 nodes as well as large graphs containing 20K-80K nodes using the same model architecture and obtained SOTA or near-SOTA results in both cases.\\
%\item 
(ii) Our model can smoothly transit from supervised learning domain to semi-supervised learning domain only by adding an extra component in the loss function, keeping the model architecture same. We applied our model for supervised tasks where number of known labels of nodes or edges in the training set is much larger or at least similar to the test set, and semi-supervised tasks where number of known labels in the training set is much less than the test set, producing SOTA or near-SOTA results for both the tasks.
%\end{enumerate}
}

==> Latex/sections/results.tex <==
%\subsection{Dataset}
%\label{ss:dataset}
\input{Latex/sections/datasets}


\begin{comment}
\subsection{Research Questions}
\label{ss:rqs}
As discussed in Section~\ref{ss:intro}, the rapid growth of graph data in different domains such as social networks, chemistry, biomedical, IoT, etc. has necessitated a generalized graph analysis framework that can work well with data belonging to different domains. In this context, we raise our first research question.

\begin{itemize}
    \item \madhu{\textbf{RQ-1}: How effectively can our proposed novel encoder-decoder based framework generalize its performance across diverse domains of graph datasets?}
\end{itemize}

\madhu{As mentioned in paragraph~\ref{super}, when dealing with large graphs in graph analysis tasks, a typical issue arises.  The utilization of one hot encoding as initial node attributes becomes unfeasible due to restricted resources, such as insufficient RAM capacity, that are required to process the entire computational graph. In context to that we investigate our second research question,}

\begin{itemize}
    \item \textbf{RQ-2}:\madhu{How efficiently can we integrate our novel supernode initialization strategy into our proposed framework to conduct experiments in a low-resource scenario, thereby achieving SOTA performance?}
\end{itemize}

\madhu{It is an important thing to discuss that how well a generalized framework, performs in constraint scenario . In context to that we investigate our third research question,}

\begin{itemize}
    \item \textbf{RQ-3}: \madhu{How well does our proposed framework perform in zero-shot scenario or in cross-domain scenario?}
\end{itemize}
\end{comment}

==> Latex/sections/subsections/expt_res_depars.tex <==
% Given an unlabelled dependency tree of a sentence (i.e. only links between tokens), the model is trained to predict the edge-labels of the tree (i.e., dependency types). From the Penn Treebank dataset, 39,680 sentences were taken for training set (with batch-size 256 and learning-rate 0.005) and 2,415 sentences were taken for test set. Initial node features are created by concatenating 100 dimensional GloVe\cite{pennington-etal-2014-glove} embedding of the tokens and 100 dimensional POS-tag embeddings. POS-tag embeddings (total 45 different POS-tags present) are initialized to random vectors $f_{POS}=[p_0, p_1, \dots , p_{99}], p_i\in[0,1] \forall i\in[0,99]$. Overall accuracy achieved was 0.87 on the test-set.

==> Latex/sections/subsections/expt_res_recoms.tex <==
 
% The task of rating prediction on the MovieLens-100k dataset is presented as a regression problem because of the fact that the rating ``4" is more similar to rating ``5" than to rating ``1", but classification problems cannot consider this fact. Commonly used performance metric for model evaluation on this dataset is RMSE loss. 80,000 edges were used as training set with LR 0.005 and the rest (20,000 edges) were kept for testing. 

To showcase the generalization ability of our proposed framework, we also investigate its performance on the movie recommendation task on the MovieLens-100k dataset. It is to be noted that in literature  movie recommendation task is considered as a regression problem since the rating ``4" is more similar to rating ``5" than to rating ``1", but classification problems do not consider this fact. Commonly used performance metric for model evaluation on this
dataset is RMSE loss. MovieLens-100k dataset contains 100,000 edges (user ratings), out of which 80,000 edges were used as training set with learning rate 0.005
and the rest (20,000) were treated as test instances. Here, the initial node features were comprised of a concatenation of various one-hot-encoded user characteristics, including user occupation (21 dimensions), user gender (2 dimensions), and user age (1 dimension). Additionally, the initial node features included information on the movie genre (19 dimensions), movie release year (1 dimension), and ratings (1-5) received from users (943 dimensions) (with a default value of 0). Furthermore, the initial node features contained ratings (1-5) given to movies (1682 dimensions) (with a default value of 0). As a result, the initial node features were quite extensive, totaling 2669 dimensions. 

Table \ref{tab:MovieLens_compare} compares the performance of our model in terms of RMSE loss to other well known models and shows that our model produces comparable results in the movie recommendation task on the MovieLens-100k dataset.
\input{Latex/Tabledef/recoms_res_cmp_tab}

==> Latex/sections/subsections/expt_res_relext.tex <==
% Given a dependency tree of a sentence, the model learns to predict the relation along with the direction between two given entities using this dataset. 8,000 annotated samples were used as the training set with batch size 1,080 and LR 0.005 and the rest (2,717 samples) were used as the test set. Total number of different types of dependency relations present in the dependency trees of the sentences in the complete dataset was 51. Considering directions along with the relation type, there was total 19 different directed relation types in the dataset. While creating batch in each epoch, 60 samples were taken from each directed relation type. There was no sample for one relation type (with direction) in the training set. For multi-word token entities, only last word was used as the entity since multiple words are different nodes in the dependency tree.

% Experiments were done using 300 dimensional GloVe\cite{pennington-etal-2014-glove} embeddings and 768 dimensional BERT\cite{kenton2019bert} embeddings of the tokens in the sentences as initial node features, separately. One hot encodings of incoming and outgoing dependency types for each token obtained from the dependency tree (51*2 = 102 dimensional) were concatenated with the GloVe and BERT embeddings, making the initial node features 402 dimensional for first case and 870 dimensional for the second case. Using GloVe embeddings, the test set accuracy was 0.73 and using BERT embeddings, the test set accuracy was 0.67.
